The homology of the stable non-orientable mapping class group

Combining results of Wahl, Galatius--Madsen--Tillmann--Weiss and Korkmaz one can identify the homotopy-type of the classifying space of the stable non-orientable mapping class group $N_\infty$ (after plus-construction). At odd primes p, the F_p-homology coincides with that of $Q_0(HP^\infty_+)$, but at the prime 2 the result is less clear. We identify the F_2-homology as a Hopf algebra in terms of the homology of well-known spaces. As an application we tabulate the integral stable homology of $N_\infty$ in degrees up to six. As in the oriented case, not all of these cohomology classes have a geometric interpretation. We determine a polynomial subalgebra of $H^*(N_\infty ; F_2)$ consisting of geometrically-defined characteristic classes.

==> chap3.tex <==
\subsection{A note on strategy}

The strategy is to apply the Eilenberg--Moore spectral sequence with $\bF_2$-coefficients to the fibrations \ref{MTO2Seq} and \ref{MTO1Seq} and in each case show that the second map ($\bar{\partial}$ or $\partial$) induces a surjection in $\bF_2$-homology. By the change-of-rings theorem for $\Cotor$ it follows that the spectral sequences collapse, and we obtain short exact sequences of Hopf algebras.

